AutoDecoding Latent 3D Diffusion Models

We present a novel approach to the generation of static and articulated 3D assets that has a 3D autodecoder at its core. The 3D autodecoder framework embeds properties learned from the target dataset in the latent space, which can then be decoded into a volumetric representation for rendering view-consistent appearance and geometry. We then identify the appropriate intermediate volumetric latent space, and introduce robust normalization and de-normalization operations to learn a 3D diffusion from 2D images or monocular videos of rigid or articulated objects. Our approach is flexible enough to use either existing camera supervision or no camera information at all -- instead efficiently learning it during training. Our evaluations demonstrate that our generation results outperform state-of-the-art alternatives on various benchmark datasets and metrics, including multi-view image datasets of synthetic objects, real in-the-wild videos of moving people, and a large-scale, real video dataset of static objects.

==> source/Figures/diffrf-cmp.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=1\textwidth]{media/diffrf-cmp.pdf} 
  \vspace{-1em}
  \caption{\small{Comparison between our method and DiffRF~\cite{mueller2022diffrf} on small-scale synthetic datasets.}}
  \label{fig:diffrf_compare} 
\end{figure*}


==> source/Sections/introduction-2.tex <==
\section{Introduction}
\label{sec:intro}

Photorealistic generation is undergoing a period that future scholars may compare to the enlightenment era. The improvements in quality, composition, stylization, resolution, scale, and manipulation capabilities of images were unimaginable just over a year ago. The abundance of online images, often enriched with text, labels, tags, and sometimes per-pixel segmentation, has significantly accelerated such progress.
The emergence and development of denoising diffusion probabilistic models (DDPMs)~\cite{sohl2015dpm_thermo,yangNEURIPS2019_3001ef25,ho2020dpm} propelled advances in image synthesis~\cite{nichol2021improveddmp,song2021scorebased,vahdat2021score,song2021denoising,dhariwal2021diff-img1,dockhorn2022score, Rombach_2022_CVPR,Karras2022edm,xiao2022DDGAN} and other domains, \eg audio (\cite{chen2021wavegrad,Forsgren_Martiros_2022,zhu2022discrete}) and video (\cite{harvey2022flexible,yin2023nuwaxl,voleti2022MCVD,ho2022video,he2023latent,mei2023vidm}). 

However, the real world is 3D, consisting of static and dynamic objects. Its geometric and temporal nature poses a major challenge for generative methods. First of all, the data we have consists mainly of images and monocular videos. For some limited categories of objects we have 3D meshes, rendered multi-view images or videos, often obtained using a tedious capturing process or created manually by artists. Second, unlike CNNs, there is no widely accepted 3D or 4D representation suitable for 3D geometry and appearance generation. As a result, with only a few exceptions~\cite{3DGP}, most of the existing 3D generative methods are restricted to a narrow range of object categories, suitable to the available data and common geometric representations. Moving, articulated objects, \eg humans, compound the problem, as the representation must also support deformations.

% The generation of realistic 3D objects relies on the ability to recognize 3D articulated representations of objects from real-world observations, be they monocular or multi-view videos or images. This seems simple at first, as it is efficiently performed by most non-predatory animals exhibiting monocular vision~\cite{Stereopsis} and certain insects~\cite{nityananda2018novel}. However, research on 3D reconstruction~\cite{PiFU,pixelNeRF} has demonstrated that modeling such behavior via machine learning techniques is challenging.

% Generative modeling requires going beyond recognizing and describing observed objects to creating plausible variations of them.
%, incorporates elements of imagination that have proven far more difficult to model algorithmically.

In this paper, we present a novel approach to designing and training denoising diffusion models for 3D-aware content suitable for efficient usage with datasets of various scales. It is generic enough to handle both rigid and articulated objects. It is versatile enough to learn diverse 3D geometry and appearance from multi-view images and monocular videos of both static and dynamic objects.
Recognizing the poses of objects in such data has proven to be crucial to learning useful 3D representations~\cite{piGAN,Chan2022,epigraf,3DGP}.
Our approach is thus designed to be robust to the use of ground truth poses, those estimated using structure-from-motion, or using no input pose information at all, but rather learning it effectively during training. It is scalable enough to train on single- or multi-category datasets of large numbers of diverse objects suitable for synthesizing a wide range of realistic content.

% Our key insight is that geometry, appearance and articulation can be not only be \emph{reconstructed} solely using 2D observations, but that, with an appropriate representation and training techniques, such reconstructions enable learning to \emph{generate} 3D content with the same supervision.
Our key insight is that, with an appropriate representation and training techniques, the capacity to \emph{reconstruct} specific geometry, appearance, and articulation from 2D observations enables the effective \emph{generation} of 3D content with only the same supervision.
We aim to learn such a representation suitable for wide-ranging content, \eg rigid or objects for which only sparse view- and motion-coverage is available. 

To this end, we define an \emph{autodecoder}~\cite{GLO,siarohin2023unsupervised,lolnerf} to learn this shared embedding space for all the objects. To sample new objects from the latent space we perform diffusion in one of the early stages of our volumetric autodecoder, shortly after the 1D embedding vector is transformed into a low-resolution latent feature volume. The compactness of this space provides the necessary regularization for geometry, allowing the training data to contain only sparse observations of each object. 

% After training, when generating samples from this latent feature volume, the autodecoder transforms and upsamples them into higher-resolution volumes containing the density and appearance information needed to render images of the content from arbitrary novel viewpoints, as during the autodecoder training process. 

As in recent diffusion techniques for image synthesis~\cite{Rombach_2022_CVPR}, our approach consists of two stages: learning a compact latent space, then using it for denoising diffusion training. Conventional approaches use an auto\emph{encoder} to learn the latent space. Diffusion sampling is then performed on the bottleneck of the autoencoder.
To learn a 3D autoencoder, one requires 3D supervision, which limits the supported object categories to those for which such supervision is available~\cite{mueller2022diffrf,cheng2023sdfusion}. The auto\emph{decoder} framework, in contrast, does not require 3D supervision to learn the 3D latent space. Instead, during training it learns a 1D embedding vector for each object in the training set. It then upsamples the 1D latent to a radiance field in which the target objects are canonically aligned, by gradually increasing the resolution of the latent volume. With this formulation we remove the requirement of the \emph{autoencoder}-based 3D diffusion methods to have 3D supervision.
Furthermore, by learning the poses of separate regions of articulated objects such as humans, we can align them in this canonical frame, then apply motion to the generated subjects for controllable animation.
% It is the autodecoder framework that enables training of 3D diffusion models with only 2D supervision.

After training the first stage, in contrast to~\cite{Rombach_2022_CVPR}, we can apply diffusion at any resolution in the autodecoder framework.
We observed that low-resolution latent spaces were too compact to generate novel objects outside the training data. The deeper layers, on the other hand acted like upsamplers. Furthermore, running diffusion sampling on high resolution volumes is costly. We found the optimal trade-off between efficiency and quality in the mid-resolution range.

We demonstrate the versatility and scalability of our approach on various tasks of rigid and articulated 3D synthesis. We first train our model using multi-view images and cameras on a setting similar to DiffRF~\cite{mueller2022diffrf} for generating shapes of a limited number of object categories. We then scale our model to hundreds of thousands of diverse objects and train using the real-world MVImgNet~\cite{yu2023mvimgnet} dataset, which is beyond the reach of prior 3D diffusion methods. 
Finally, we train our model on a subset of CelebV-Text~\cite{yu2022celebvtext}, consisting of $\sim$44K sequences of high quality videos.


==> source/Sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}

{\color{red}\makeatletter\let\default@color\current@color\makeatother

  open w/ a captivating and relevant quote? some ideas/examples:

  ``In photography there is a reality so subtle that it becomes more real than reality.''
  — Alfred Stieglitz

  ``The photograph itself doesn’t interest me. I want only to capture a minute part of reality.''
  — Henri Cartier-Bresson

  ``Taking an image, freezing a moment, reveals how rich reality truly is.''
  — Anonymous

  ``A photograph is usually looked at - seldom looked into.''
  - Ansel Adams

  more examples: https://petapixel.com/photography-quotes/, https://www.pixpa.com/blog/quotes-about-photography
}

\textit{
% Creation and consumption of content have always been integral aspects of our cultural evolution.
Since the oral narratives shared around communal fires, prehistoric cave paintings in France, and the dramatic masterpieces of ancient Greece, human beings have expressed their stories in diverse and multifaceted ways.
Over time, content creation and consumption have undergone a process of commodification, with innovations such as Gutenberg's printing press, radio, magazines and television bringing increasingly intricate forms of entertainment into our daily lives.
The next frontier to be explored involves the commodification of three-dimensional (3D) entertainment through Augmented and Virtual Reality technologies.}

\textit{Recent breakthroughs in Artificial Intelligence have enabled the automated generation of content in textual (e.g., ChatGPT, BART) and visual (e.g., DALL-E, StableDiffusion, ImaGEN) domains, made possible by training on extensive datasets. In this study, we endeavor to advance large-scale 3D content generation, bringing this cutting-edge field one step closer to realization.}

Many of the long-standing and most challenging open problems in modern computer vision \red{and machine learning?} ultimately represent a fundamental human desire to fully understand how the information depicted in images and videos -- short and simple glimpses of a specific time and place -- capture and describe the content of the world well enough to recreate, change, and control this content, and even to create new variations and extensions of this content inspired by reality, but which presently only exist in our minds.
While our memories and imaginations allow us to exploit a lifetime of observations to perform such tasks, envisioning variations of what we've seen that can often be described in only a few common words, communicating such thoughts in detail from one person to another, however, requires translating them into some shareable representation.

This is easier said than done.
2D and 3D modeling and animation tools and techniques are cumbersome, time-consuming, and labor-intensive, requiring talent and years of expertise and training to create complex and detailed content, making them intractable for most novices and casual users. % for more than trivial copy-pasting pre-existing assets lacking plausible variety.
Thus, even simple tasks for an average individual, such as imagining a random person nodding their head or an everyday object, seen consistently from multiple viewpoints, results in thoughts not easily and accurately conveyed to others.

Recent developments in generative modeling demonstrates impressive progress towards these ends, enabling the easy creation and control of varying, complex, and detailed depictions of novel objects and scenes. %, drawn from combinations and variations of the key shared and distinguishing features extracted from the provided training data.
In particular, the introduction and development of denoising diffusion probabilistic models (DDPMs)~\cite{sohl2015dpm_thermo,yangNEURIPS2019_3001ef25,ho2020dpm} led to work making impressive improvements the state-of-the-art in both conditional and unconditional image synthesis~\cite{nichol2021improveddmp,song2021scorebased,vahdat2021score,song2021denoising,dhariwal2021diff-img1,dockhorn2022score, Rombach_2022_CVPR,Karras2022edm,xiao2022DDGAN} and other domains, \eg audio (\cite{chen2021wavegrad,Forsgren_Martiros_2022,zhu2022discrete}) and video (\cite{harvey2022flexible,yin2023nuwaxl,voleti2022MCVD,ho2022video,he2023latent,mei2023vidm}).
However, extending such approaches to controllable, high-quality generation and animation of 3D content is quite challenging.

Of particular concern is the type of supervision needed for such tasks, as directly using existing 3D content is intuitive, but in fact quite limiting.
Aside from the question of how to adapt existing approaches to an appropriate representation of 3D shape and appearance, existing datasets of either manually-generated synthetic models or 3D reconstructions of real objects and scenes have issues concerning the quality, complexity, realism, and variety of the content, particularly for openly accessible datasets.
For dynamic, non-rigid 3D objects, these issues are compounded by the absence of large-scale 3D datasets containing the animation parameters for dynamic, non-rigid 3D objects with enough diversity to plausibly generate and animate such variations in both content and motion.
As such, well-curated datasets of appropriate 3D content are relatively small for generative tasks.

% However, extending these models to the controllable generation of 3D content suitable for high-fidelity rendering and animation is quite challenging.
% Tractably adapting existing architectures and training techniques for image or video generation to this domain is not trivial, especially as suitable 3D content representations (\eg meshes, voxels, point clouds, or implicit neural representations) each have their own advantages and disadvantages.
% Furthermore, supervision with existing 3D content datasets is intuitive but in fact quite limiting.
% Synthetic, artist-generated 3D assets, which vary in quality and scale for open datasets (and cost, accessibility, and legality for closed datasets), lack photorealism, and few have animation controls needed to plausibly generate dynamic objects and creatures.
% Datasets of 3D reconstructions of real-world geometry and appearance from image or video datasets require extensive computation to create, and the results vary in accuracy, noise, occlusions, and variety of subjects.
% Moving content such as people must also be omitted (for static reconstructions) or specially handled (for dynamic reconstructions, \eg of humans).
% As such, the scale and feasibility of these datasets limits their applicability to generative modeling.

The abundance of real-world 2D images and videos suggests a promising alternative, as learning to render such images allows for indirectly learning the underlying structure and appearance of image content.
Recent work~\cite{siarohin2023unsupervised} demonstrated the utility of volumetric rendering techniques for unsupervised animation of faces and bodies learned from large-scale 2D video sequences.
By estimating the appearance, geometry, and non-rigid motion of these subjects, and then aligning them within a canonical pose in a 3D space, an autodecoder can be trained to generate these volumetric representations from a compact embedding vector corresponding to each training subject.
The estimated motion can then be transferred from one embedded subject to another, then rendered to perform plausible performance retargeting and 3D-aware novel view synthesis.
However, this approach does not allow for plausible or controllable generative sampling of new subjects.
Nor does it show the capacity to learn effective 3D content from sparse multi-view images rather than videos, or to generalize to more than one object category when training a model.

% drawn from combinations and variations of the key shared and distinguishing features extracted from the provided training data.

In this work, we introduce a new approach to designing and training denoising diffusion models for 3D-aware content generation, rendering, animation, and manipulation, designed for efficient usage with datasets of widely varying scales. %, by employing latent diffusion in a compact 3D space, coupled with volumetric autodecoders trained using a rendering consistency loss with images from the target dataset.
% \textbf{3D} \textbf{V}olumetric \textbf{A}uto-\textbf{D}ecod\textbf{ER}s.
Our key insight is that using an autodecoder model that employs latent 3D content representations as described above, supervised by volumetric rendering, coupled with an appropriate latent 3D diffusion training process, addresses the aforementioned challenges and limitations of prior work. % by allowing for efficient diffusion training and sampling within a low-dimensional, latent volumetric space.
This diffusion is performed in one of the early stages of our volumetric autodecoder, shortly after the $1$D embedding vector is transformed into a low-resolution latent feature volume.
The compactness of this space allows for efficient and scalable training on input from various domains, while retaining high quality in the sampled content.
After training, when generating samples from this latent feature volume, the autodecoder transforms and upsamples them into higher-resolution volumes containing the density and appearance information needed to render images of the content from arbitrary novel viewpoints, as during the autodecoder training process.

% The use of such a flexible content representation and rendering process allows for .

Ours is the first work, to our knowledge, capable of performing 3D structure and appearance generation, using only 2D supervision from images or videos, which enables various tasks ranging from conditional and unconditional generation to controllable animation of non-rigid content.
We demonstrate its capabilities with a variety of datasets and input modalities, including sparse, multi-view images of both real and synthetic objects, and short, continuous video sequences of real, moving human subjects.
The number of unique objects in our datasets range from fewer than $1.7$K to $300$K, and include both single- and multi-category object datasets, demonstrating the capacity of our approach to widely varying datasets at vastly different scales.
We show state-of-the-art results on unconditional generation of the images and corresponding geometry, using multiple benchmarks and metrics employed by prior works.

Interestingly, while prior works training 3D diffusion models for generation primarily focus on a specific input modality, \eg sparse multi-view images of static objects or continuous video sequences, we find that our approach works for \emph{both} of these modalities, including in the challenging case in which our rendering is supervised with imperfectly estimated camera poses relative to non-rigid subjects such as humans in motion.
Furthermore, As no domain-specific priors for pose, motion, appearance is required for this work, it can be easily applied not only to large-scale 2D human datasets, but also to arbitrary target domains, including datasets with widely varying object categories.
% Furthermore, this work demonstrated impressive results for the task of performance retargeting by optimizing an embedding of the source subject's appearance and transferring the estimated motion from the driving subject to it.
% However, its ability to generate subjects with new appearances with controllable poses and motion by sampling from the embedding space makes it a promising framework for tasks, \eg conditional and non-conditional object generation without domain-specific priors.
\kyle{Remove next line if we cannot demonstrate this in the results.}
\red{Furthermore, we demonstrate that this approach allows for both conditional and unconditional content generation, enabling text-conditioned synthesis.}

In summary, our primary contributions are as follows:

\begin{itemize}

    \item A novel approach to 3D content generation with denoising diffusion models, extending them to the latent 3D space of volumetric autodecoders trained with only 2D supervision;

    \item Crucial enhancements to state-of-the-art autodecoding and diffusion modeling techniques, enabling their combined application to 3D content generation suitable for high-fidelity rendering and training on datasets with drastically diverse scales and content;

    \item Extensive qualitative and quantitative evaluations of our content generation and rendering results on various datasets, including both real videos of non-rigid people and sparse multi-view image collections, as well as on both real and synthetic content;

    \item Analysis and ablations of the key aspects of our approach and the essential design choices for our network architectures and training procedures; and

    \item Demonstations of various applications using the generated objects, including consistent 3D-aware novel view synthesis, surface mesh extraction, \red{and} motion transfer with controllable viewpoints for generating and animating dynamic humans\red{, and both conditional and unconditional content generation}.

\end{itemize}

The remainder of the paper is organized as follows: Sec.~\ref{sec:related_work} reviews the related work in 3D generative models, denoising diffusion models, and neural rendering techniques for content generation and manipulation.
Sec.~\ref{sec:method} describes our proposed methodology, including design choices enabling our architecture and training process to address diverse object categories, datasets, and tasks.
Sec.\ref{subsec:method_volum_autodecoding} explains the architecture of our volumetric autodecoder, and how it is trained to infer the 3D geometry and appearance needed to render and animate content from the target dataset.
Sec.\ref{subsec:method_diff_3d} illustrates the latent 3D diffusion training process enabling this model to generate 3D content with novel appearance and geometry by sampling from the autodecoder's latent space.
Sec.~\ref{sec:results} presents qualitative and quantitative results from our experiments; comparisons on benchmarks and multiple diverse datasets of varying scales; and an ablation study evaluating and validating our design choices (\ref{subsec:results_ablation}).
Finally, Sec.~\ref{sec:conclusion} presents our final conclusions and insights gained from this work.

% (Secs.~\ref{subsec:method_training}-~\ref{subsec:method_inference});

\kyle{TODO: add note saying whether code/models will be made publicly available?}


==> source/Tables/old_ablation.tex <==
\begin{wrapfigure}[16]{r}{0.5\textwidth}
% \begin{table}[t]

\caption{\textbf{3D Autodecoder Ablation.}
% To evaluate the effectiveness of our components, we start with the vanilla version of our autodecoder architecture for voxel generation. 
``-'' indicates this component has been removed. As we remove each sequentially, the final row depicts results for the unmodified architecture and training procedure. LPIPS results are multiplied by $10^2$.
}
% \vspace{-2mm}
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lcc}
\cmidrule[1.0pt]{1-3}
Model  & PSNR~$\uparrow$ & LPIPS~$\downarrow$ \\
\cmidrule[1.0pt]{1-3}
Ours &  \textbf{27.719} & \textbf{6.255} \\
\cmidrule[1.0pt]{1-3}
~~-~Multi-Frame Training & 27.176 & 6.855 \\
~~-~Self-Attention      &  27.335  & 6.738 \\
%~~-~Foreground Loss & 27.335 & 6.718  \\
~~-~Increased Depth  & 27.24 & 6.924  \\
~~-~Embedding Length ($1024\rightarrow64$) & 25.985 & 8.332 \\
\cmidrule[1.0pt]{1-3}
\cmidrule[1.0pt]{1-3}
\end{tabular}
}
\vspace{-1mm}
\label{tab:ablation}

% \end{table}
\end{wrapfigure}


==> source/Tables/old_sota3d.tex <==
\begin{table}[t]
\centering
\resizebox{.95\columnwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
 & \multicolumn{2}{c}{PhotoShape Chairs~\cite{photoshape2018}} & \multicolumn{2}{c}{ABO Tables~\cite{collins2022abo}} \\
Method  & FID $\downarrow$ & KID $\downarrow$ & FID $\downarrow$ & KID $\downarrow$ \\
\midrule
$\pi$-GAN~\cite{piGAN}      &  52.71  &  13.64  &  41.67  &  13.81 \\
EG3D~\cite{Chan2022}                         &  16.54  &  8.412  &  31.18  &  11.67 \\
\red{DiffRF~\cite{mueller2022diffrf} w/o 2D} &  18.27  &  9.263  &  35.89  &  13.94 \\
DiffRF~\cite{mueller2022diffrf}              &  15.95  &  \textbf{7.935}  &  27.06 &  10.03 \\
\midrule
Ours    & \textbf{15.82} & 8.688 & \textbf{18.44} & \textbf{6.854} \\
\bottomrule
\end{tabular}
}
\caption{\textbf{Quantitative comparison} of unconditional generation on the PhotoShape Chairs~\cite{photoshape2018} and ABO Tables~\cite{collins2022abo} datasets. Our method achieves a better image generation quality than state-of-the-art GAN-based approaches, and DiffRF, which uses diffusion with 3D and 2D supervision. \red{DiffRF's optional 2D rendering loss improves the results substantially, but our method still outperforms it overall.} KID scores are multiplied by $10^3$.
\kyle{Maybe we should re-add the DiffRF w/o 2D supervision (red above). It shows ours is better by a larger margin when they don't have 3D \emph{and} 2D supervision by each image metric, and that the results w/ other 2D only methods are sometimes better than DiffRF w/ just 3D, but still worse overall than ours.}}
\label{tab:sota3d}
\end{table}

